A Discontinuous Galerkin Method for Ideal Two-Fluid Plasma Equations

A discontinuous Galerkin method for the ideal 5 moment two-fluid plasma system is presented. The method uses a second or third order discontinuous Galerkin spatial discretization and a third order TVD Runge-Kutta time stepping scheme. The method is benchmarked against an analytic solution of a dispersive electron acoustic square pulse as well as the two-fluid electromagnetic shock and existing numerical solutions to the GEM challenge magnetic reconnection problem. The algorithm can be generalized to arbitrary geometries and three dimensions. An approach to maintaining small gauge errors based on error propagation is suggested.

==> divergence-errors.tex <==
\subsection{Divergence errors}
Divergence errors are a common problem in plasma codes and techniques
for solving these issues have been discussed in detail for 
magnetohydrodynamics codes in \cite{Toth2000}.  Ultimately divergence cleaning will 
need to be applied to the two-fluid plasma algorithm.  However, our experience has
shown that the discontinuous Galerkin method applied to the two-fluid plasma
system works quite well without divergence cleaning in cases where a finite volume
code (developed in parallel) fails completely.

Two techniques have been applied to the
finite volume method that can also be applied to the discontinuous Galerkin algorithm for
the two-fluid system.  The first method solves the potential form of Maxwell's equations
re-written as a system of 16 first order equations.  In this case, both divergence
constraints are satisfied automatically though a new constraint, the Lorentz gauge condition for example,
arises.  Since the gauge condition is first order, gauge cleaning may be performed algebraically for each cell.  A second
approach to divergence cleaning, which has been used successfully by the authors in the
the finite volume code, is to use the perfectly hyperbolic Maxwell's equations as described
in \cite{Munz2000}.  Both these techniques are hyperbolic divergence cleaning techniques
so they can be applied to the described algorithm simply by changing $Q_{em}$, $F_{em}$ and
$\psi_{em}$ if Lax fluxes and componentwise limiting is used.  If Riemann fluxes or characteristic
limiting is used then the eigensystems of the new electromagnetic systems would also need
to be calculated.  

In MHD codes large divergence errors can occur at shocks, in the two-fluid
plasma system this is not such an issue since true shocks do not occur in the magnetic field.
For most situations, true shocks only occur in the ion fluid, followed by a smooth Debye length transition
in the electron quantities and then a broader transition in the magnetic field field profile.  
Finally, the results of this research have benefited from the parallel
development of a divergence cleaned finite volume two-fluid code \cite{Hakim2005} so that results
could be compared.


==> electrostatic-plasma-shock.tex <==
\subsection{Two-Fluid Electrostatic Plasma Shock}
In this section we include a simulation of a simple gas dynamic shock using the two-fluid equations.  
The electrons and ions start out with the same discontinuous
pressure and number density profile.  The solution is allowed to evolve in time.  The domain
size is 10,000 cells in the simulation takes 200,000 time steps.  An electrostatic 
field is quickly generated which couples the ions to the electrons.  Parameters used are, $q_{i}=10$, $q_{e}=-10$, $m_{i}=1$, $m_{e}=\frac{1}{1836}$,
$\epsilon_{0}=1$, $\mu_{0}=1$, $c=1$, $\gamma_{e}=\gamma_{i}=\frac{5}{3}$.
For a comparison, a neutral fluid with the same mass density as the ions and double 
the ion pressure is also included.  The initial
conditions are,
\begin{equation}
	\left(
	\begin{array}{c}
	n_{e}\\
	U_{e\,x}\\
	U_{e\,y}\\
	U_{e\,z}\\
	P_{e}\\
	n_{i}\\
	U_{i\,x}\\
	U_{i\,y}\\
	U_{i\,z}\\
	P_{i}\\
	B_{x}\\
	B_{y}\\
	B_{z}\\
	E_{x}\\
	E_{y}\\
	E_{z}\\
	\end{array}
	\right)_{left}=
	\left(
	\begin{array}{c}
	1.0\\
	0\\
	0\\
	0\\
	0.5\times 10^{-4}\\
	1.0\\
	0\\
	0\\
	0\\
	0.5\times 10^{-4}\\
	0\\
	0\\
	0\\
	0\\
	0\\
	0\\
	\end{array}
	\right),\quad \text{and} \quad
	\left(
	\begin{array}{c}
	n_{e}\\
	U_{e\,x}\\
	U_{e\,y}\\
	U_{e\,z}\\
	P_{e}\\
	n_{i}\\
	U_{i\,x}\\
	U_{i\,y}\\
	U_{i\,z}\\
	P_{i}\\
	B_{x}\\
	B_{y}\\
	B_{z}\\
	E_{x}\\
	E_{y}\\
	E_{z}\\
	\end{array}
	\right)_{right}=
	\left(
	\begin{array}{c}
	0.125\\
	0\\
	0\\
	0\\
	0.05\times 10^{-4}\\
	0.125\\
	0\\
	0\\
	0\\
	0.05\times 10^{-4}\\
	0\\
	0\\
	0\\
	0\\
	0\\
	0\\
	\end{array}
	\right)\,.
\end{equation}
These initial conditions give a Debye length $\lambda_{d}=\frac{v_{th\,e}}{w_{p\,e}}=1\times 10^{-3}$ based on the conditions
on the left hand side of the domain. 
The electric field in the two-fluid solution
couples the electron and ion pressures so that the shocks in the two-fluid solution match the location of the 
shocks in the neutral fluid solution.  There remain significant differences in the two-fluid and neutral fluid solutions.  
In figure \ref{F:GDFull} spikes in ion density appear in the two-fluid solution on the Debye length scale.  
The spike at the shocks has a simple physical explanation and is commonly seen in simulations of partially ionized gases\cite{Auslender2000}.  
The electric field increases
the speed of the ion shock to match the speed of the neutral shock.  The ion conditions at the ion shock still have 
to satisfy the Rankine Hugoniot relations, so roughly a Debye
length before the shock the ions adjust their jump conditions to produce a shock that has the neutral fluid shock speed.  
As a result, in figure \ref{F:GDRight}
a smooth rise in the ion density is seen just before the ion shock.  The jump conditions at 
the ion shock produce a shock speed given by the neutral fluid shock speed to one percent.  
 
The waves that appear at 
the base of the rarefaction wave (close up in figure \ref{F:GDLeft}) can be explained in a similar manner though roughly 80 percent
of the magnitude of the spikes is a result of errors in Poisson's equation.  
The neutral rarefaction wave moves faster than the ion rarefaction wave by itself.  The ion fluid attempts to
undergo rarefaction before the electron fluid, when this happens an electric field develops which pulls the ion fluid
density back to the electron fluid density.   This process is repeated until the ions and electrons form a rarefaction wave
at the same point fig.\ref{F:GDLeft}, which also is the same point that the neutral solution rarefies at.  
The shocks themselves disappear if Poisson's equation is enforced and are replaced by smooth transitions.  

As a practical matter these Debye length oscillations may disappear when
electron-ion collisional effects or other collisional effects are included in the code; however, similar 
effects have been observed in simulations of partially ionized gases \cite{Auslender2000}
and the existence of ion subshocks are discussed in \cite{Kennel85} for example.  Nevertheless, 
the analysis is important because Debye length oscillations routinely appear in 
two-fluid simulations and the effects are not always numerical.  At the base of rarefactions, un-resolved Debye length
leads to large errors in Poisson's equation and significant charge separation on a scale much 
greater than the Debye length; the effect is to artificially increase the Debye length.  
To avoid this problem, the grid spacing should approximately resolve the Debye length.

The two-fluid solution differs from the neutral solution in the pressure profile as well.  In fig.\ref{F:GDPressure}
the electron and ion pressures differ in the region between the contact discontinuity and the shock wave in such
a manner that the electron pressure is decreased by roughly the same amount that the ion pressure is increased.  This
indicates that the pressure difference occurs because of an electric field due to charge separation, this charge imbalance begins
with a negative charge bump at the base of the rarefaction and is resolved with the positive charge spike at the shock.  The electric
field supports a fluid pressure gradient which is exactly opposite for the electrons and ions.
The pressure solution between the contact discontinuity and the shock remains unchanged when Poisson's equation is enforced, i.e.,
the two-temperature effect is not numerical.
\begin{figure}%\label{F:GDFull}
	\begin{center}
	\scalebox{0.6}{\includegraphics{gddensityfull.eps}}
	\end{center}%\label{F:GDFull}
	\caption{Plot of number density vs position for the electron and ion fluid in comparison with a single
	fluid for the electrostatic plasma shock.
	The two-fluid equations behave much like a single fluid in this case except in the vicinity of
	the shocks where the ion fluid number density increases and in the region right of the rarefaction wave
	where similar number density variations occur.  The spike at the shock remains un-changed when electric field
	divergence cleaning is applied, but the spikes at the rarefaction wave decrease in amplitude significantly (though never
	disappear) when electric field divergence cleaning is implemented.}\label{F:GDFull}
\end{figure}%\label{F:GDFull}
\begin{figure}
	\begin{center}
	\scalebox{0.6}{\includegraphics{gddensityright.eps}}
	\end{center}\label{F:GDRight}
	\caption{Plot of number density vs position in comparison with the single fluid solution close to the shock in the electrostatic plasma shock problem.
	The ion fluid density increases near the shock so that the jump condition is satisfied (the solution remains unchanged when Poisson's equation
	is enforced).  Debye shielding occurs around this spike in charge density (the Debye length is $2.4\times 10^{-3}$ in this region) 
	and the single fluid solution lies within this Debye shielding region.}\label{F:GDRight}
\end{figure}
\begin{figure}
	\begin{center}
	\scalebox{0.6}{\includegraphics{gddensityleft.eps}}
	\end{center}
	\caption{Plot of two-fluid number densities compared to the single fluid solution close to the rarefaction wave in the electrostatic shock problem.
	The oscillations in ion density occur because the ion fluid attempts to form a rarefaction wave before the electron fluid.  The result is
	a series of rarefaction like bumps.  In the plots above, when Poisson's equation is not enforced the small rarefactions end in shock waves.
	When Poisson's equation is enforced the shocks disappear being replaced by a smooth transition the bumps shrink in amplitude by about 80 percent.  
	Note that the charge separation is occurring on Debye length scales (the Debye length is $1.1\times 10^{-3}$ in this region).}\label{F:GDLeft}
\end{figure}
\clearpage
\begin{figure}%\label{F:GDPressure}
	\begin{center}
	\scalebox{0.6}{\includegraphics{gdpressurefull.eps}}
	\end{center}
	\caption{Plot of pressure vs position for the electron and ion fluid in comparison with a single fluid.  Notice
	that between the location of the contact discontinuity and the shock the electron and ion pressures are different.
	This pressure difference is a result of the electric field generated at the base of the contact discontinuity due to
	charge separation in that region.  The charge separation disappears in a short distance, but the effect on the pressure
	remains until the shock is reached.}\label{F:GDPressure}
\end{figure}

